Structural Attention: Rethinking Transformer for Unpaired Medical Image Synthesis

Unpaired medical image synthesis aims to provide complementary information for an accurate clinical diagnostics, and address challenges in obtaining aligned multi-modal medical scans. Transformer-based models excel in imaging translation tasks thanks to their ability to capture long-range dependencies. Although effective in supervised training settings, their performance falters in unpaired image synthesis, particularly in synthesizing structural details. This paper empirically demonstrates that, lacking strong inductive biases, Transformer can converge to non-optimal solutions in the absence of paired data. To address this, we introduce UNet Structured Transformer (UNest), a novel architecture incorporating structural inductive biases for unpaired medical image synthesis. We leverage the foundational Segment-Anything Model to precisely extract the foreground structure and perform structural attention within the main anatomy. This guides the model to learn key anatomical regions, thus improving structural synthesis under the lack of supervision in unpaired training. Evaluated on two public datasets, spanning three modalities, i.e., MR, CT, and PET, UNest improves recent methods by up to 19.30% across six medical image synthesis tasks. Our code is released at https://github.com/HieuPhan33/MICCAI2024-UNest.

==> src/related_works.tex <==
\section{Related Works}
\textbf{Image-to-image translation} (I2I) aims to synthesize an image in a target domain from a source domain. %Variational autoencoders (VAEs)~\cite{kingma2013auto} and generative adversarial networks (GANs)~\cite{goodfellow2020generative} are the two most approaches commonly employed to model the distribution of the target domain and produce convincing `fake' data. VAE methods~\cite{kingma2013auto,liu2018constrained} convert data points into a probabilistic latent space and then recreate them from samples of latent distributions. GANs~\cite{goodfellow2020generative}, on the other hand, formulate the learning process as a minimax competition, where the generator is trained to deceive the discriminator by generating authentic-seeming data points, while the discriminator aims to differentiate between the actual and generated samples. GANs are expressive and flexible models having the ability to produce high-resolution, diverse, and style-distinct images~\cite{abdal2019image2stylegan,skorokhodov2022stylegan}.
%Generative adversarial networks (GANs)~\cite{goodfellow2020generative} are among the most common approaches used to model the distribution of the target domain and produce convincing `fake' data. %It produces high-resolution and diverse images for a variety of synthesis tasks such as image segmentation~\cite{kalluri2022cluster}, super-resolution~\cite{wang2018esrgan,zhang2019multiple}, image registration~\cite{zheng2021symreg} and medical image translation~\cite{dalmaz2022resvit,ge2019unpaired,yang2020unsupervised}. %I2I is first introduced in Pix2Pix~\cite{isola2017image}, which is a type of conditonal GAN. It uses a generator $G$, consisting of an encoder and a decoder, to transform an image from one domain to another. 
Pix2Pix~\cite{isola2017image} and subsequent works~\cite{wang2019drpan,park2019semantic,zhu2020sean} %such as DRPAN~\cite{wang2019drpan}, SPADE~\cite{park2019semantic}, and SEAN~\cite{zhu2020sean} 
assume the source and target domains have paired data and adopt a supervised training paradigm. %Despite their ability to generate realistic images, unpaired I2I is more desirable because acquiring paired data is expensive in most settings. 
CycleGAN~\cite{zhu2017unpaired} and U-GAT-IT~\cite{kim2019u} are pioneering works in unpaired I2I by exploiting a cycle consistency loss. They train two generators to enforce an image to be consistent after a cycle of translation. To preserve structures after translation, many methods incorporate instance-level knowledge~\cite{mo2018instagan,kim2022instaformer} or attention mechanisms~\cite{tang2021attentiongan}. Notably, AttentionGAN~\cite{tang2021attentiongan} includes an attention branch to differentiate background and foreground objects, thus enabling translation without altering the background.  Instead of using bidirectional mapping, several methods~\cite{park2020contrastive,zheng2021spatially,jung2022exploring,hu2022qs} exclude cycle-consistency loss and apply contrastive loss between image patches to enforce an alternative structural consistency. %They introduce structural consistency by applying a patch-level contrastive loss between the original and translated images.  %Instead of bidirectional mappings in CycleGAN framework, several methods only trains a single $G$ to perform one-direction mappings. They incorporate structural consistency using contrastive loss between important patches of the original and the translated images. 
%CUT~\cite{park2020contrastive} is a pioneer work, which applies contrastive loss between features of the original and the translated image at random locations. 

%They perform contrastive learning on more meaningful locations by mining hard negative samples via pixel-wise similarities~\cite{jung2022exploring} or using attention mechanisms~\cite{hu2022qs}. %A recent technique~\cite{jung2022exploring} uses semantic similarity between pixels to mine hard negative examples for the feature contrastive learning. The QS-Attention~\cite{hu2022qs} uses global/local self-attention to select key features based on entropy calculations on the attention matrix, subsequently applying contrastive loss between these important features in the source and target domain for feature alignments across domains. %QS-Attention~\cite{hu2022qs} computes global/local self-attention and queries a subset of important features based on the entropy computed on a row of the attention matrix. It routes the values to learn features for important queries and then apply contrastive loss between important features between the source and target domain. 
%While these approaches save training memory by employing only one generator, 
%These methods can be less desirable when the need for generating both domains is crucial, especially in cases of imputing missing modalities in medical applications.
%Based on how the sources of information are leveraged, I2I can be grouped into three categories. Supervised I2I approaches such as Pix2Pix~\cite{isola2017image}, DRPAN, SPADE~\cite{park2019semantic}, and SEAN~\cite{zhu2020sean} assume the data from two domains are \textit{paired} and directly optimize the supervised loss to minimize the discrepancy between the synthetic image and the ground truth. Unpaired I2I methods, on the other hand, leverage \textit{unpaired} sets of training images to learn the mappings. These methods differ in how they devise the loss objective to enable training without pairings. CycleGAN~\cite{zhu2017unpaired} is a pioneering work in an unsupervised setting. It proposes a cycle consistency loss which minimizes the reconstruction error when a translated image is reverted to the original image. Extending CycleGAN, U-GAT-IT~\cite{kim2019u} employs more advanced generator and discriminator networks to enhance its performance.

% Recent methods apply unidirection mapping and incorporate structural consistency using contrastive loss between important patches of the original and the translated images. CUT~\cite{park2020contrastive} is the first work proposed to apply contrastive loss between features of the original and the translated image on the same location. It uses the encoder extracted from the first half of the generator for feature extraction. Several works exploit the feature relations to incorporate second-order statistics into their contrastive learning paradigm. Notably, F-SLE~\cite{zheng2021spatially} use patch-wise similarity maps for contrastive loss. A recent technique~\cite{jung2022exploring} uses semantic similarity between pixels to mine hard negative examples for the feature contrastive learning. QS-Attention~\cite{hu2022qs} computes global/local self-attention and queries a subset of important features based on the entropy computed on a row of the attention matrix. It routes the values to learn features for important queries and then apply contrastive loss between important features between the source and target domain. 

\textbf{Medical image synthesis} is a specific application of I2I in the medical domain, which has been widely used to estimate missing modalities~\cite{fei2022classification}, create annotated datasets~\cite{costa2017end}, improve image segmentation~\cite{li2020towards}, and enable image super-resolution~\cite{yang2023deep}. Most synthesis techniques use a paired I2I framework to perform MRI-to-CT~\cite{emami2021sa,zhang2022map}, PET-to-CT~\cite{armanious2020medgan}, and MRI synthesis~\cite{cao2020auto}. %Auto-GAN~\cite{cao2020auto} uses a self-representation network to learn features of a target domain and applies knowledge distillation to encourage the feature alignment between the generator and the self-representation network.
%CycleGAN~\cite{zhang2022map} trains four generator networks to perform bidirectional PET-CT mappings in both image and sinogram domains. To ensure model converge, they require paired data to perform the initial supervised learning stage to ensure network convergence. 
%Despite generating high-quality images, these methods require training on a large-scale paired dataset, which is prohibitively expensive to acquire. 

Several studies apply CycleGAN's framework for unsupervised MRI-to-CT synthesis, such as~\cite{yang2020unsupervised, liu2021ct, ge2019unpaired,kong2021breaking}. However, these methods often underperform when compared to supervised approaches. They rely on convolution (conv) operators, whose receptive fields are restricted, lacking the ability to learn global contexts. Conv-based synthesis methods are known to suffer from atypical anatomy~\cite{dalmaz2022resvit} and are suboptimal in learning long-range dependencies~\cite{wang2018non}. Many methods augment Conv-based architectures by incorporating self-attention modules for PET synthesis~\cite{lan2021three}, CT denoising~\cite{li2020sacnn} or liver MR enhancement~\cite{zhao2020tripartite}. %3D conditional GAN method~\cite{lan2021three} applies a self-attention module to extract global features and perform PET synthesis from low-dose PET images. Similarly, SA-CNN~\cite{li2020sacnn} introduces a 3D self-attention module, combined with a self-supervised learning scheme, to denoise low-dose CT scans. 
%Tripartite-GAN~\cite{zhao2020tripartite} incorporates a dual-attention module that simultaneously learns spatial and channel dependencies for enhancing the contrast of liver MR scans. The majority of attention-based methods follow supervised learning paradigm and require paired data. 

%\textbf{Transformer methods for I2I.} Most methods design hybrid Conv-Transformer architectures.  CyTran~\cite{ristea2023cytran} and UVCGAN~\cite{torbunov2023uvcgan}, as pioneering works in unpaired training, incorporate Transformer blocks in convolution-based generators for medical and natural image synthesis, respectively. In related research, ResViT~\cite{dalmaz2022resvit} designs a Transformer block with a residual convolutional connection for \textit{paired} medical image synthesis. Exploiting contextual learning, many methods insert Transformer layers between the encoder and the decoder for image segmentation~\cite{chen2021transunet}, image super-resolution~\cite{feng2021task}, CT denoising~\cite{wang2021ted}, and image reconstruction~\cite{luo20213d,korkmaz2022unsupervised}. Nevertheless, their core feature extractor is convolutional layers, limiting model expressiveness in learning global contexts. 
\textbf{Transformer methods for I2I.} Most methods design hybrid Conv-Transformer architectures. A recent method, ResViT~\cite{dalmaz2022resvit}, designs a Transformer block with a residual convolutional connection for paired medical image synthesis. Exploiting contextual learning, many methods insert Transformer layers between the encoder and the decoder for image segmentation~\cite{chen2021transunet}, image super-resolution~\cite{feng2021task}, CT denoising~\cite{wang2021ted}, and image reconstruction~\cite{luo20213d,korkmaz2022unsupervised}. Cytran~\cite{ristea2023cytran} and UVCGAN~\cite{torbunov2023uvcgan} stand as pioneering works in applying hybrid models to unpaired training for medical and natural image synthesis, respectively. They incorporate Transformer blocks in convolution-based generators. However, the core feature extractors of hybrid methods still rely on convolutional operators, limiting model expressiveness in fully capturing contextual features.

Several methods apply a pure Transformer architecture for \textit{paired} MR synthesis~\cite{zhang2022ptnet3d} and medical image segmentation~\cite{hatamizadeh2022unetr,tang2022self,huang2022miss,cao2022swin,lin2022ds}. 
%UNETR~\cite{hatamizadeh2022unetr} and SwinUNETR~\cite{tang2022self} propose a pure Transformer encoder to effectively extract contextual feature for medical image segmentation. 
Notably, UNETR~\cite{hatamizadeh2022unetr} and PTNet~\cite{zhang2022ptnet3d} eliminate the convolution-like inductive bias and apply global attention to the entire image. Without strong biases, they struggle to converge when applied to unpaired image synthesis. Swin UNETR~\cite{tang2022self} and DS-TransUNet~\cite{lin2022ds} introduce local inductive bias by performing attention within a small window. While segmentation only assigns discrete labels, image synthesis produces continuous intensity values for every anatomical region, spanning from smooth brain tissue to structural bone details. Current methods with restricted local attention can miss important contexts within the anatomical structures. This paper is the first work designing a pure Transformer with structural attention for effective unpaired medical image synthesis. %proposes to introduce structural priors into Transformer, guiding the attention within the main anatomy for unpaired medical image synthesis.  % Show some 

%To effectively capture contextual representations, pure Transformer methods have received greater attention in various medical applications such as image segmentation~\cite{chen2021transunet,xie2021cotr}, reconstruction~\cite{luo20213d}, registration~\cite{chen2022transmorph} and image translation~\cite{dalmaz2022resvit}. ResViT~\cite{dalmaz2022resvit} is a recent technique that [...] for generic paired medical image synthesis.



==> tab/att-abl.tex <==
\begin{table}[!h]
    \centering
    \resizebox{0.47\textwidth}{!}{%
    \begin{tabular}{@{}cc||cccccc@{}}
    \toprule 
    \multirow{2}{*}{FG} & \multirow{2}{*}{BG} & \multicolumn{2}{c}{PET-CT} & \multicolumn{2}{c}{MR-CT} & \multicolumn{2}{c}{MR-PET} \\\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}
    &  & MAE$\downarrow$ & SSIM$\uparrow$ & MAE$\downarrow$ & SSIM$\uparrow$ & MAE$\downarrow$ & SSIM$\uparrow$  \\\midrule
    \multicolumn{2}{c||}{Global} & 10.91 & 75.88 & 7.84 & 81.23 & 7.33 & 81.96   \\
    \multicolumn{2}{c||}{Local} & 10.82 & 75.97 & 8.12 & 81.06 & 7.64  & 81.53  \\
    \midrule
    Struct & Struct & 9.73 & 77.85 & 6.97 & 83.75 & 7.05 & 82.09 \\
    %Local & Struct & 10.80 & 75.91  & 7.90 & 81.15 & 7.38 & 81.77  \\
    Struct & Local  & \textbf{9.57} & \textbf{78.47} & \textbf{6.18} & \textbf{85.48} & \textbf{6.32} & \textbf{82.97} \\\bottomrule
    \end{tabular}%
    }
    \caption{Accuracies on three tasks using different attention mechanisms for foreground (FG) and background (BG).}
    \label{tab:abl-att}
\end{table}
%% Why does global attention is effective for brain scans
%% The amount of smoother regions in brain are denser than whole-body scans => Local context is less effective

==> tab/mask-abl.tex <==

\begin{table}[!h]
    \centering
    \resizebox{0.4\textwidth}{!}{%
    \begin{tabular}{@{}cc||cc|cc@{}}
        \toprule
        \multirow{2}{*}{Mask gen.} & \multirow{2}{*}{$N_{\text{mask}}$} & \multicolumn{2}{c}{PET-CT} & \multicolumn{2}{c}{MR-CT}\\ 
        \cmidrule(lr){3-4} \cmidrule(lr){5-6}
        & & MAE & SSIM & MAE & SSIM \\
        \midrule
        \multicolumn{2}{c||}{Global attention} & 10.95 & 75.88 & 7.84 & 81.23 \\
        \midrule
        Img. proc. & 3000 & 10.23 & 76.39 & 7.38  & 82.75 \\
        SAM & 3000 & 9.57 & 78.47 & 6.18 & 85.48 \\
        \midrule
        SAM & 0 & 10.67 & 75.96 & 7.75 & 81.30 \\
        SAM & 1000 & 9.91 & 77.56 & 6.53 & 84.76 \\
        SAM & 5000 & 9.60 & 78.23 & 6.26 & 85.11\\
        \bottomrule
    \end{tabular}
    }
    \caption{Performance using different algorithms to generate ground-truth masks (mask gen.) with different values of $N_{\text{mask}}$. Img. proc.: image processing techniques. $N_{\text{mask}}$: number of training iterations before using prediction from patch classifier instead of the ground-truth masks. Our gains mainly arise from a structural inductive bias, without depending on optimal masks from the large SAM model. When $N_{\text{mask}}=0$, the model's performance drops. This indicates unstable training when directly using predicted masks $M$ before the patch classifier is trained properly.}
    \label{tab:abl}
\end{table}

==> tab/pet-ct.tex <==
\begin{table}[!h]
    \centering
    \begin{tabular}{@{}lccc||ccc@{}}
    \toprule \multirow{ 2}{*}{\textbf{Methods}} & \multicolumn{3}{c}{\textbf{PET-to-CT}} & \multicolumn{3}{c}{\textbf{CT-to-PET}} \\
         & MAE $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & MAE $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$  \\\midrule
         \textit{Convolution-based} \\ \midrule
         CycleGAN~\cite{zhu2017unpaired} & 14.34 & 32.30 & 66.85 & 12.80 & 31.95 & 69.53 \\
    % MedGAN~\cite{armanious2020medgan} & { 32.54 & {32.57 & {52.67 & {30.87 & {31.45 & {50.57\\
         sc-CycleGAN~\cite{yang2020unsupervised} & {14.59} & {32.42} & {67.43} & {12.77} & {32.05} & 70.53 \\
         %shape-CycleGAN~\cite{ge2019unpaired} & {26.98} & {30.12} & {62.25} & {27.96} &{30.27} & {60.88} \\
AttentionGAN~\cite{tang2021attentiongan} & {13.62} &{32.97} & {67.12} & {11.87}  &{32.61} & 72.54 \\
         QS-Attention~\cite{hu2022qs} & {13.21}  & {33.70} & 71.49 & 9.75 & 33.21 & 77.42 \\
          \midrule
         \textit{Hybrid Convolution-Transformer} \\ \midrule 
        TransUNet~\cite{chen2021transunet} & 16.65 & 32.68 & 62.68 & 13.52 &  31.94 & 67.88  \\
        Cytran~\cite{ristea2023cytran} & 14.77 & 32.24 & 64.37 & 9.05 & 33.56 & 74.65 \\ % Apply Transformer on high-level features struggle to synthesize high-res CT from a low-res PET scan
        %UVCGAN~\cite{torbunov2023uvcgan} & 13.88 & 32.75 & 66.29 & 9.55 & 32.88 & 72.45 \\ % Apply Transformer on high-level features struggle to synthesize high-res CT from a low-res PET scan
         ResViT (Dalmaz et al. 2022) & 13.55 & 33.28 & 70.53 & 9.90 & 32.13 & 68.29  \\
         \midrule
         \textit{Pure Transformers} \\ \midrule
         PTNet~\cite{zhang2022ptnet3d} & 14.11 & 32.62 & 66.53 & 9.24 & 32.77 & 70.53 \\
         UNETR~\cite{hatamizadeh2022unetr} & 11.08 & 33.70 & 76.06 & 7.77 & 33.58 & 80.30 \\
         Swin-UNETR~\cite{tang2022self} & 10.93 & 33.78 & 76.42 & 7.42 & 33.78 & 80.53 \\
         \midrule
         UNest (Ours) & \textbf{9.57}  & \textbf{34.05} & \textbf{78.47} & \textbf{6.55} & \textbf{34.27} & \textbf{81.55} \\\hline
    \end{tabular}
        \caption{Quantitative comparison of different methods on the AutoPET dataset for translating between PET and CT. The improvement of UNest over all compared methods is statistically significant at $p=0.05$. The standard deviation is reported in Suppl. due to space constraints.}
    \label{tab:sota-pet-ct}
\end{table}
